A Unified Analysis of Saddle Flow Dynamics: Stability and Algorithm Design

This work examines the conditions for asymptotic and exponential convergence of saddle flow dynamics of convex-concave functions. First, we propose an observability-based certificate for asymptotic convergence, directly bridging the gap between the invariant set in a LaSalle argument and the equilibrium set of saddle flows. This certificate generalizes conventional conditions for convergence, e.g., strict convexity-concavity, and leads to a novel state-augmentation method that requires minimal assumptions for asymptotic convergence. We also show that global exponential stability follows from strong convexity-strong concavity, providing a lower-bound estimate of the convergence rate. This insight also explains the convergence of proximal saddle flows for strongly convex-concave objective functions. Our results generalize to dynamics with projections on the vector field and have applications in solving constrained convex optimization via primal-dual methods. Based on these insights, we study four algorithms built upon different Lagrangian function transformations. We validate our work by applying these methods to solve a network flow optimization and a Lasso regression problem.

==> ack.tex <==
% use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...

==> edits_pcyou.tex <==
% \usepackage{ifthen}
% \newboolean{showcomments}
% \setboolean{showcomments}{true}
% \usepackage[usenames,dvipsnames]{xcolor}
% %\usepackage{todonotes}
% \usepackage{soul}

% \definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
% \definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}

% %ADD CITES
% \newcommand{\addcite}[0]{\ifthenelse{\boolean{showcomments}}
% {\textcolor{purple}{(add cite(s)) }}{}}%

% % Comments
% % \newcommand{\pcyou}[1]{  \ifthenelse{\boolean{showcomments}}
% % {\todo[inline,color=bleudefrance]{PCY: #1}}{}}
% % \newcommand{\emmargin}[1]{\ifthenelse{\boolean{showcomments}}{\marginpar{\color{bleudefrance}\tiny PCY: #1}}{}}
% % \newcommand{\emumargin}[1]{  \ifthenelse{\boolean{showcomments}}
% % {\todo[color=bleudefrance,size=\tiny]{PCY: #1}} {}}

% % \makeatletter
% % \if@todonotes@disabled
% % \newcommand{\hlfix}[2]{\hl{#1}}
% % \else
% % \newcommand{\hlfix}[2]{\hl{#1}\todo[color=bleudefrance,size=\tiny]{PCY: #2}}
% % \fi
% % \makeatother


% %\usepackage{comment}
% \newcommand{\slow}[1]{\ifthenelse{\boolean{showcomments}}
% 	{ \textcolor{red}{(SL:  #1)}}{}}
% \newcommand{\you}[1]{\ifthenelse{\boolean{showcomments}}
% 	{ \textcolor{blue}{(PCY:  #1)}}{}}
% \newcommand{\john}[1]{\ifthenelse{\boolean{showcomments}}
% 	{ \textcolor{green}{(jp:  #1)}}{}}


% %Edits to be highlighted
% \newboolean{showedits}
% \setboolean{showedits}{true}
% \usepackage[xcolor=bleudefrance]{changes}
% \definechangesauthor[color=bleudefrance]{PCY}
% \newcommand{\aem}[1]{
% \ifthenelse{\boolean{showedits}}
% {\added[id=PCY]{#1}}
% {#1}
% }
% \newcommand{\chem}[2]{
% \ifthenelse{\boolean{showedits}}
% {\replaced[id=PCY]{#1}{#2}}
% {#1}
% }
% \newcommand{\dem}[1]{
% \ifthenelse{\boolean{showedits}}
% {\deleted[id=PCY]{#1}}
% {}
% }
% %\listoftodos[{\color{red}\textbf{List of comments/suggestions}}]

\usepackage[utf8]{inputenc}
\usepackage{epsfig, latexsym, times, bbm}
\usepackage{color}
\usepackage{colortbl}
\usepackage{array}
\usepackage{cite}
\usepackage{amsmath}
%\usepackage{graphics}
\usepackage{graphicx}
%\usepackage{epstopdf}
\usepackage{amssymb}
\usepackage{url}
%\usepackage{comment}
%\usepackage{caption}
\usepackage{multirow}
\def\UrlBreaks{\do\/\do-}
%\captionsetup{justification   = raggedright, singlelinecheck = false}
\usepackage{bbding}
\usepackage{amsfonts}
\usepackage{cases}
%\usepackage{caption}
\usepackage{subfigure}
%\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{mathrsfs}
\usepackage{bm}
\usepackage{verbatim}
\usepackage{enumerate}
%\usepackage[colorlinks,
%            linkcolor=black, % ref, red
%            anchorcolor=black, % bookmark, blue
%            citecolor=black % cite, green
%            ]{hyperref}
\usepackage{booktabs}
\usepackage[linesnumbered,ruled,longend]{algorithm2e}
\usepackage{textcomp}
%% mac unsupported
%\usepackage{slashbox}
\usepackage{subeqnarray}
\usepackage{amsthm}
\DeclareGraphicsExtensions{.pdf,.jpeg,.png,.es,.jpg,.eps}
\graphicspath{{figures/}}





%% added
\def\ba{\begin{array}}
	\def\ea{\end{array}}
\newcommand{\beq}{\begin{equation}}
	\newcommand{\eeq}{\end{equation}}
\newcommand{\bq}{\begin{eqnarray}}
	\newcommand{\eq}{\end{eqnarray}}
\newcommand{\bqn}{\begin{eqnarray*}}
	\newcommand{\eqn}{\end{eqnarray*}}
\newcommand{\bee}{\begin{enumerate}}
	\newcommand{\eee}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
	\newcommand{\ei}{\end{itemize}}
\newcommand{\bseq}{\begin{subequations}}
\newcommand{\eseq}{\end{subequations}}
%\newcommand{\qed}{\hfill{$\blacksquare$}}
\newcommand{\ii}{\textbf{i}}
\newcommand{\diag}{\textrm{diag}}
\newcommand{\blockdiag}{\textrm{blockdiag}}

% \newtheorem{definition}{\textbf{Definition}}
% \newtheorem{assumption}{\textbf{Assumption}}
% \newtheorem{proposition}{\textbf{Proposition}}
% \newtheorem{corollary}{\textbf{Corollary}}
% \newtheorem{lemma}{\textbf{Lemma}}
% \newtheorem{theorem}{\textbf{Theorem}}
% \newtheorem{remark}{\textbf{Remark}}



\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}
\newcommand{\cell}[3]{\parbox[c][#2][c]{#1}{\makebox[#1]{#3}}}

\renewcommand\thepage{}
\renewcommand{\arraystretch}{1.3}

% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}
\allowdisplaybreaks

\usepackage{enumitem}
% \setlist{leftmargin=15pt,labelindent=15pt}
% \setlist[enumerate]{align=left}

\setlist[enumerate]{leftmargin=*,label=\arabic*.}
\setlist[itemize]{leftmargin=*}
% \setlist[enumerate]{
%   align=left,
%   labelwidth=1.5em,
%   labelsep=0pt,
%   leftmargin=1.5em,
%   label=\arabic*.,
% }
